TrimTuner: Efficient Optimization of Machine Learning Jobs in the Cloud via Sub-Sampling

This work introduces TrimTuner, the first system for optimizing machine learning jobs in the cloud to exploit sub-sampling techniques to reduce the cost of the optimization process while keeping into account user-specified constraints. TrimTuner jointly optimizes the cloud and application-specific parameters and, unlike state of the art works for cloud optimization, eschews the need to train the model with the full training set every time a new configuration is sampled. Indeed, by leveraging sub-sampling techniques and data-sets that are up to 60x smaller than the original one, we show that TrimTuner can reduce the cost of the optimization process by up to 50x. Further, TrimTuner speeds-up the recommendation process by 65x with respect to state of the art techniques for hyper-parameter optimization that use sub-sampling techniques. The reasons for this improvement are twofold: i) a novel domain specific heuristic that reduces the number of configurations for which the acquisition function has to be evaluated; ii) the adoption of an ensemble of decision trees that enables boosting the speed of the recommendation process by one additional order of magnitude.

==> biblio.tex <==

IEEEexample.bib 
V1.13 (2008/09/30)
Copyright (c) 2002-2008 by Michael Shell
See: http://www.michaelshell.org/
for current contact information.

This is an example BibTeX database for the official IEEEtran.bst
BibTeX style file.

Some entries call strings that are defined in the IEEEabrv.bib file.
Therefore, IEEEabrv.bib should be loaded prior to this file.
Usage:

\bibliographystyle{./IEEEtran}
\bibliography{./IEEEabrv,./IEEEexample}


Support sites:
http://www.michaelshell.org/tex/ieeetran/
http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
and/or
http://www.ieee.org/

*************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEabrv.bib, IEEEfull.bib, IEEEexample.bib,
                   IEEEtran.bst, IEEEtranS.bst, IEEEtranSA.bst,
                   IEEEtranN.bst, IEEEtranSN.bst, IEEEtran_bst_HOWTO.pdf
*************************************************************************
% MTBO
@inproceedings{mtbo,
    author = {Swersky, Kevin and Snoek, Jasper and 	Adams, Ryan P.},
    title = {Multi-task Bayesian Optimization},
    booktitle = {NIPS},
    year = {2013},
    volume = {2},
    location = {Lake Tahoe, Nv, USA},
    pages = {2004--2012},
} 
%Proceedings of the 26th International Conference on Neural Information Processing Systems},


% BO
@techreport{boTutorial,
    Author = {Eric Brochu and Vlad M Cora and Nando {de                  Freitas}},
    Number = {arXiv:1012.2599},
    Title = {A Tutorial on Bayesian Optimization of Expensive          Cost Functions, with Application to Active User            Modeling and Hierarchical Reinforcement Learning},
    Year = {2010}}
}

@article{Jones:1998,
    author = {Jones, Donald R. and Schonlau, Matthias and                Welch, William J.},
    title = {Efficient Global Optimization of Expensive                 Black-Box Functions},
    journal = {J. of Global Optimization},
    year = {1998},
    volume = {13},
    number = {4},
    pages = {455--492},
    publisher = {Kluwer Academic Publishers},
} 


% TL 
@article{tlSurvey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on knowledge and data engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2009},
  publisher={IEEE}
}

@inproceedings{tl,
  title={Transfer learning for performance modeling of configurable systems: An exploratory analysis},
  author={Jamshidi, Pooyan and Siegmund, Norbert and Velez, Miguel and K{\"a}stner, Christian and Patel, Akshay and Agarwal, Yuvraj},
  booktitle={2017 32nd IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={497--508},
  year={2017},
  organization={IEEE}
}

% ES
@inproceedings{entropySearch,
  title={Entropy Search for Information-Efficient Global Optimization},
  author={Henning, Philipp and Schuler, Christian J.},
  booktitle={Journal of Machine Learning Research},
  volume={13},
  number={Jan},
  pages={1809--1837},
  year={2012},
}

@inproceedings{Kullback-Leibler_divergence, 
    author = {S. Kullback and R. A. Leibler},
    title = {On Information and Sufficiency},
    booktitle = {The Annals of Mathematical Statistics},
    Volume = {22},
    Number = {1},
    year = {1951}, 
    pages = {79-86},
}

%PES
@inproceedings{pes,
    author = {Hern\'{a}ndez-Lobato, Jos\'{e} Miguel and Hoffman, Matthew W. and Ghahramani, Zoubin},
    title = {Predictive entropy search for efficient global optimization of black-box functions},
    booktitle = {Proceedings of the 27th International Conference on Neural Information Processing Systems},
    volume={1},
    year = {2014},
    location = {Montreal, Canada},
    pages = {918-926},
}

%pesc
@inproceedings{pesc,
    author = {Hern\'{a}ndez-Lobato, Jos\'{e} and Gelbart, Michael and Hoffman, Matthew and Adams, Ryan and Ghahramani, Zoubin},
    year = {2015},
    pages = {1699-1707},
    title = {Predictive Entropy Search for Bayesian Optimization with Unknown Constraints},
    booktitle = {ICML},
    location = {Lille, France},
}
%Proceedings of the 32nd International Conference on International Conference on Machine Learning


%mes
@InProceedings{mes,
  title = {Max-value Entropy Search for Efficient {B}ayesian Optimization},
  author ={Zi Wang and Stefanie Jegelka},
  booktitle ={Proceedings of the 34th International Conference on Machine Learning},
  pages = {3627--3635},
  year = {2017},
  volume = {70},
  location = {Sydney, Australia},
  publisher = {PMLR},
}

%cmes
@article{cmes,
    author = {Valerio Perrone and Iaroslav Shcherbatyi and Rodolphe Jenatton and C{\'e}dric Archambeau and Matthias Seeger},
    title = {Constrained Bayesian Optimization with Max-Value Entropy Search},
    journal   = {ArXiv},
    volume = {abs/1910.07003},
    year = {2019}
}


% BOHB
@InProceedings{bohb,
  title = 	 {{BOHB}: Robust and Efficient Hyperparameter Optimization at Scale},
  author = 	 {Falkner, Stefan and Klein, Aaron and Hutter, Frank},
  booktitle = 	 {ICML},
  pages = 	 {1437--1446},
  year = 	 {2018},
  volume = 	 {80}
}
%Proceedings of the 35th International Conference on Machine Learning},

% ProteusTM
@inproceedings{proteustm,
    author = {Didona, Diego and Diegues, Nuno and Kermarrec,             Anne-Marie and Guerraoui, Rachid and Neves,                Ricardo and Romano, Paolo},
    title = {ProteusTM: Abstraction Meets Performance in                Transactional Memory},
    booktitle = {ASPLOS},
    year={2016},
    location = {Atlanta, GA, USA},
} 

% FABOLAS
@inproceedings{fabolas,
    title={Fast Bayesian Optimization of Machine Learning Hyperparamaters on Large Datasets},
    author={Klein, Aaron and Falkner, Stefan and Bartels, Simon and Hennig, Philipp and Hutter, Frank},
    booktitle={AISTATS},
    volume={54},
    pages={528--536},
    year={2017},
}
%publisher = {PMLR},
%Proceedings of the 20th International Conference on Artificial Intelligence and Statistics}


% Hyperband
@article{hyperband,
    author = {Li, L. and Jamieson, K. and DeSalvo, Giulia and Rostamizadeh, A. and Talwalkar, A.},
    year = {2018},
    pages = {1-52},
    title = {Hyperband: A novel bandit-based approach to hyperparameter optimization},
    volume = {18},
    journal = {Journal of Machine Learning Research}
}

% CherryPick
@inproceedings{cherrypick,
    author = {Alipourfard, Omid and Liu, Hongqiang Harry and             Chen, Jianshu and Venkataraman, Shivaram and Yu,           Minlan and Zhang, Ming},
    title = {Cherrypick: Adaptively Unearthing the Best Cloud            Configurations for Big Data Analytics},
    booktitle = {NSDI},
    year={2017}
}

% Arrow
@inproceedings{arrow,
    author    = {Chin{-}Jung Hsu and
               Vivek Nair and
               Vincent W. Freeh and
               Tim Menzies},
    title     = {Arrow: Low-Level Augmented Bayesian                     Optimization for Finding the Best Cloud {VM}},
    booktitle = {ICDCS},
    year = {2018},
    location  = {Vienna, Austria}
}

% Lynceus
@inproceedings{lynceus,
    author    = {Casimiro, Maria and Didona, Diego and Romano, Paolo and Rodrigues, Luís and Zwanepoel, Willy and Garlan, David},
    title     = {Lynceus: Cost-efficient Tuning and Provisioning of Data Analytic Jobs},
    booktitle   = {ICDCS},
    year      = {2020},
}

% Scout
@article{scout,
    title={Scout: An Experienced Guide to Find the Best Cloud          Configuration},
    author={Hsu, Chin-Jung and Nair, Vivek and Menzies, Tim and         Freeh, Vincent W},
    journal={arXiv preprint arXiv:1803.01296},
    year={2018},
}

% Tensorflow
%Barham, Paul and Chen,              Jianmin and Chen, Zhifeng and Davis, Andy and              Dean, Jeffrey and Devin, Matthieu and Ghemawat,            Sanjay and Irving, Geoffrey and Isard, Michael             and Kudlur, Manjunath and Levenberg, Josh and              Monga, Rajat and Moore, Sherry and Murray, Derek           G. and Steiner, Benoit and Tucker, Paul and                Vasudevan, Vijay and Warden, Pete and Wicke,               Martin and Yu, Yuan and Zheng, Xiaoqiang},
@inproceedings{tensorflow,
    author = {Abadi, Mart\'{\i}n and others},
    title = {TensorFlow: A System for Large-scale Machine Learning},
    booktitle = {OSDI},
    year={2016},
    location = {Savannah, GA, USA},
} 

% WEKA
@article{weka,
    author = {Hall, Mark and Frank, Eibe and Holmes, Geoffrey            and Pfahringer, Bernhard and Reutemann, Peter              and Witten, Ian H.},
    title = {The WEKA Data Mining Software: An Update},
    journal = {SIGKDD Explorations Newsletter},
    volume = {11},
    number = {1},
    year = {2009},
    publisher = {ACM},
}

% MNIST dataset
@inproceedings{mnist,
  title={The MNIST database of handwritten digit images for machine learning research [Best of the Web]},
  author={Deng, Li},
  booktitle={IEEE Signal Processing Magazine},
  volume={29},
  number={6},
  year={2012},
  organization={IEEE},
}


%information theory -> entropy
@article{info_theory,
  author = {Shannon, Claude E.},
  journal = {Bell Syst. Tech. J.},
  number = 3,
  pages = {379-423},
  title = {A mathematical theory of communication.},
  volume = 27,
  year = 1948
}


%BO, gps hyperparameters->marginalize over GPs with MCMC
@inproceedings{Practical_BO,
    author = {Snoek, Jasper and Larochelle, Hugo and P. Adams, Ryan},
    title = {Practical Bayesian Optimization of Machine Learning Algorithms},
    booktitle = {NIPS},
    volume = {2},
    year = {2012},
    location = {Lake Tahoe, Nv, USA},
    pages = {2951--2959},
}
%Proceedings of the 25th International Conference on Neural Information Processing Systems}


%matern 5/2 kernel
@book{matern,
  title={Spatial Variation},
  author={Matérn, Bertil},
  year={1986},
  publisher={Springer-Verlag},
  address = {Berlin, Germany},
}

@INPROCEEDINGS{gaussianprocesses,
    author = {Michael A. Osborne and Roman Garnett and Stephen J. Roberts},
    title = {Gaussian processes for global optimization},
    booktitle = {LION},
    year = {2009}
}

%%%%%%%%% LATIN HYPERCUBE SAMPLING %%%%%%%%%%%%

@inproceedings{LHS,
    author = { Michael   Stein },
    title = {Large Sample Properties of Simulations Using Latin Hypercube Sampling},
    booktitle = {Technometrics},
    volume = {29},
    number = {2},
    pages = {143-151},
    year  = {1987},
}


@inproceedings{LHS_original,
    author = {M. D. McKay and R. J. Beckman and W. J. Conover},
    booktitle = {Technometrics},
    number = {2},
    pages = {239-245},
    volume = {21},
    year = {1979},
}

@inproceedings{eic,
    author = {Gardner, Jacob R. and others},
    title = {Bayesian Optimization with Inequality Constraints},
    booktitle = {ICML},
    year={2014}
}

@inproceedings{ei,
    title={The Application of Bayesian Methods for Seeking the Extremum},
    author={Mockus, J and Tiesis, Vytautas and Zilinskas, Antanas},
    booktitle={Toward Global Optimization},
    volume={2},
    pages={117--128},
    year={1978},
    organization = {Elsevier},
}

@inproceedings{ei2,
    author="Jones, Donald R. and Schonlau, Matthias and Welch, William J.",
    title="Efficient Global Optimization of Expensive Black-Box Functions",
    booktitle="Journal of Global Optimization",
    year="1998",
    volume="13",
    number="4",
    pages="455--492",
    organization="Springer",
}


%direct
@article{direct,
author = {Jones, D. R. and Perttunen, C. D. and Stuckman, B. E.},
title = {Lipschitzian Optimization without the Lipschitz Constant},
year = {1993},
publisher = {Plenum Press},
address = {USA},
volume = {79},
number = {1},
journal = {J. Optim. Theory Appl.},
pages = {157–181},
}


%cmaes
@Inbook{cmaes,
author="Hansen, Nikolaus",
editor="Lozano, Jose A.
and Larra{\~{n}}aga, Pedro
and Inza, I{\~{n}}aki
and Bengoetxea, Endika",
title="The CMA Evolution Strategy: A Comparing Review",
bookTitle="Towards a New Evolutionary Computation: Advances in the Estimation of Distribution Algorithms",
year="2006",
publisher="Springer Berlin Heidelberg",
pages="75--102",
}

@inproceedings{paris,
  title={Selecting the best vm across multiple public clouds: A data-driven performance modeling approach},
  author={Yadwadkar, Neeraja J and Hariharan, Bharath and Gonzalez, Joseph E and Smith, Burton and Katz, Randy H},
  booktitle={SoCC},
  pages={452--465},
  year={2017}
}
%  Proceedings of the 2017 Symposium on Cloud Computing}


@misc{aws:minute,
    author = "{Jeff Bar, AWS blog}",
    title = {{Per-Second Billing for EC2 Instances and EBS Volumes}},
    howpublished = {\url{http://tinyurl.com/ycajp922}},
    note = {accessed 4 Jan. 2020},
    year=2017,
}

@misc{azure:minute,
    author = "{Microsoft Azure}",
    title = {{Azure Billing per minute}},
    howpublished = {{\url{https://azure.microsoft.com/en-us/pricing/details/cloud-services/}}},
    note = {accessed 4 Jan. 2020} ,
    year=2018,
}

@misc{google:minute,
    author = "{Paul Nash}",
    title = {{Per second billing in Google Cloud}},
    howpublished = {{\url{https://cloudplatform.googleblog.com/2017/09/extending-per-second-billing-in-google.html}}},
    note = {accessed 4 Jan. 2020} ,
    year=2017,
}

@misc{aws:flavors,
    author = "{Amazon Web Services}",
    title = {{Amazon EC2 Instance Types}},
    howpublished = {{\url{https://aws.amazon.com/ec2/instance-types/}}},
    note = {accessed 30 Jun. 2020} ,
}


%%bagging
@Article{bagging,
    author="Breiman, Leo",
    title="Bagging Predictors",
    journal="Machine Learning",
    year="1996",
    volume="24",
    number="2",
    pages="123--140"
}

@inproceedings{ernest,
  title={Ernest: Efficient performance prediction for large-scale advanced analytics},
  author={Venkataraman, Shivaram and Yang, Zongheng and Franklin, Michael and Recht, Benjamin and Stoica, Ion},
  booktitle={NSDI},
  year={2016}
}


@INPROCEEDINGS{zengIPDPS18, 
   author={Zeng, Jingna and Romano, Paolo and Barreto, Joao and Rodrigues, Lu{\'\i}s and Haridi, Seif}, 
    booktitle={IPDPS}, 
    title={Online Tuning of Parallelism Degree in Parallel Nesting Transactional Memory}, 
    year={2018}, 
}


@article{ituned,
    author    = {Songyun Duan and
                Vamsidhar Thummala and
                Shivnath Babu},
    title     = {Tuning Database Configuration Parameters with             iTuned},
    journal   = {VLDB},
    year={2009},
    volume    = {2},
    number    = {1},
}

@inproceedings{aml19,
  author    = {Emma Strubell and
               Ananya Ganesh and
               Andrew McCallum},
  title     = {Energy and Policy Considerations for Deep Learning in {NLP}},
  booktitle = {ACL},
  year      = {2019}
}

% Quasar
@inproceedings{quasar,
    author = {Delimitrou, Christina and Kozyrakis, Christos},
    title = {Quasar: Resource-efficient and QoS-aware Cluster           Management},
    booktitle = {ASPLOS},
    year={2014}
}

@book{decisionTrees,
    title={Classification and regression trees},
    author={Breiman, Leo},
    year={1984},
    publisher={Routledge},
}

% Markov Chain Monte Carlo
@article{mcmc,
  title={A tutorial on adaptive MCMC},
  author={Andrieu, Christophe and Thoms, Johannes},
  journal={Statistics and computing},
  volume={18},
  number={4},
  pages={343--373},
  year={2008},
  publisher={Springer}
}

@article{informationgain,
  title={Information gain and a general measure of correlation},
  author={Kent, John T},
  journal={Biometrika},
  volume={70},
  number={1},
  pages={163--173},
  year={1983},
  publisher={Oxford University Press}
}


%gauss-hermite quadrature
@inproceedings{GH_quadrature,
    title={A note on Gauss-Hermite quadrature},
    author={Liu, Qing and Pierce, Donald A},
    booktitle={Biometrika},
    volume={81},
    number={3},
    pages={624--629},
    year={1994},
    organization = {Oxford University Press, Biometrika Trust},
}



@inproceedings{extraTree,
author = {Geurts, Pierre and Ernst, Damien and Wehenkel, Louis},
year = {2006},
pages = {3-42},
title = {Extremely Randomized Trees},
volume = {63},
booktitle = {Journal of Machine Learning},
doi = {10.1007/s10994-006-6226-1}
}


@article{george,
    author = {{Ambikasaran}, S. and {Foreman-Mackey}, D. and {Greengard}, L. and {Hogg}, D.~W. and {O'Neil}, M.},
    title = "{Fast Direct Methods for Gaussian Processes}",
    journal   = {ArXiv},
    volume = {abs/1403.6015},
    year = {2014}    
}

==> files/rw.tex <==
\section{Related Work}

This section describes state-of-the-art work related to \ts{}. We discuss three lines of related work: approaches for cloud optimization, approaches for hyper-parameter tuning and common acquisition functions employed in the BO setting.


\mynewpar{Cloud Optimization Approaches.}
%CherryPick
%Lynceus
%SCOUT  => TL
Recent works to find the optimal configuration to deploy jobs in the cloud, such as CherryPick~\cite{cherrypick} and Arrow~\cite{arrow} focus solely on optimizing cloud related parameters and disregard the possibility of learning from related tasks. Lynceus~\cite{lynceus} improves over these systems by jointly optimizing both application-specific and cloud parameters during the optimization process. Unfortunately, it does not account for the possibility of learning from related tasks. Further, Lynceus solves a different optimization problem: it minimizes the cost of the exploration process added with the cost of running the job in the final selected configuration. Differently, \ts{} aims at maximizing the accuracy of the job while ensuring that the user-defined constraints, either on cost or time, are complied with. Scout~\cite{scout}, although only optimizing cloud parameters similarly to CherryPick and Arrow, differs from these by leveraging transfer learning techniques to improve the quality of the configuration it recommends. However, while in Scout these techniques serve to reuse knowledge from previous optimization processes, \ts{} instead leverages such techniques to learn how the same job behaves in sub-sampled datasets of different sizes. Thus, \ts{} improves over these approaches by jointly optimizing both cloud and application-specific parameters and by taking into account knowledge from related tasks in order to reduce the cost of the optimization process.


\mynewpar{Hyper-parameter Tuning Approaches.}
%Hyperband
%BOHB
%FABOLAS
Hyperband~\cite{hyperband}, BOHB~\cite{bohb} and FABOLAS~\cite{fabolas} optimize the choice of hyper-parameters of machine learning jobs. Hyperband is a model-free approach that leverages a technique called Successive Halving~\cite{}. BOHB builds from Hyperband, but uses BO to guide the search, thus bringing together the advantages of successive halving and model based search. However, it disregards past knowledge and does not take into account the cost of the optimization process. Unlike this approach, FABOLAS leverages transfer learning techniques to decrease the overhead of the search process. Nonetheless, none of these approaches are suitable for finding the optimal cloud parameters to deploy ML jobs in the cloud. \ts{}, instead, takes into account specific idiosyncrasies characteristic of the cloud setting, thus finding optimal configurations to deploy ML jobs, while also leveraging transfer learning techniques to decrease the cost of the search process.

\mynewpar{Common Acquisition Functions.}
Typical acquisition functions in which state-of-the-art hyper-parameter and cloud optimization approaches~\cite{cherrypick,lynceus,fabolas} rely on to select the next point to sample and guide the search for the optimum are  Expected Improvement (EI)~\cite{ei,ei2}, constrained EI (EIc)~\cite{eic} or Entropy Search (ES)~\cite{entropySearch}. EI and EIc trade-off \textit{exploitation} (testing points that are considered good) and \textit{exploration} (testing uncertain points) of the search space to find the configuration that is expected to improve the most over the currently known optimum, with EIc taking into account quality of service (QoS) constraints. ES, in its turn, aims at maximizing the knowledge attained through each exploration. Additionally, there are two prominent variations of the ES function, namely Predictive Entropy Search with Constraints (PESC)
~\cite{pesc} and constrained Max-value Entropy Search (cMES)~\cite{cmes}. These variants use different approximations and techniques to compute the Entropy Search, which render the use of non-stationary kernels or decision trees, such as the ones employed by \ts{}, infeasible. As such, we could not leverage any of these acquisition functions.

%\textbf{TODO: May be this part could be discussed in related work?}
%Both co-variance functions selected correspond to non-stationary kernels. 
%Other state-of-the-art acquisition functions such as PESC \cite{pesc} and cMES \cite{cmes}, that solve similar optimization problems, use different approximations and techniques to compute the Entropy Search. However, these do not allow non-stationary kernels to be used, which help \ts{} enhance the performance of its models and thus improve the overall optimization process.

%\noindent\textbf{Popular Acquisition Functions}
%\noindent\textbf{Entropy Search (ES) Variants}
%ES
%PES
%cPES
%PESMO
%MES
%cMES
%Most state-of-the-art hyper-parameter and cloud optimization approaches rely on model-based techniques to drive the search for the optimal configuration.
%A prominent model-based technique employed by these works is Bayesian Optimization, which we describe in more detail in Section~\ref{sec:background}.
%These modelling techniques work in an iterative fashion, sequentially profiling points in order to predict the best configuration. Selecting the next point to sample requires balancing
%Typical acquisition functions in which state-of-the-art hyper-parameter and cloud optimization approaches~\cite{cherrypick,lynceus,fabolas} rely to select the next point to sample and guide the search for the optimum are  Expected Improvement (EI)~\cite{ei}, constrained EI (EIc)~\cite{eic} or Entropy Search (ES)~\cite{es}. EI and EIc trade-off \textit{exploitation} (testing points that are considered good) and \textit{exploration} (testing uncertain points) of the search space to find the configuration that is expected to improve the most over the currently known optimum, with EIc taking into account quality of service (QoS) constraints. ES, in its turn, aims at maximizing the knowledge attained through each exploration. 

%There are several variants of the ES, namely Predictive ES (PES)~\cite{pes}, PES constrained (PESC)~\cite{pesc}, %PES for Multi-Objective BO (PESMO)~\cite{pesmo}, Max-Value ES (MES)~\cite{mes} and constrained MES (cMES)~\cite{cmes}.  The difference between ES and PES resides in the approximation that is used to compute the entropy reduction due to sampling a given point. PES is based on the fact that the reduction in the entropy of the optimum $x^*$ due to evaluating $f(x)$ is equivalent to the mutual information between the $x^*$ and $f(x)$. Since the mutual information is a symmetric function, the reduction in the entropy of $x^*$ due to testing $f(x)$ is equal to the reduction in the entropy of $f(x)$ obtained by measuring $x^*$
%\begin{equation}
%    PES(x) = H[p(y|\mathcal{S},x)] - E_{p(x^*|\mathcal{S})}[H[p(y|\mathcal{S},x,x^*)]].
%    \label{eq:pes}
%\end{equation}
%The first term can be computed in the closed-form through the posterior marginals for $f(x)$ and the second term needs to be approximated as described in \cite{pes}.
%MES, instead, differs from PES because it uses the information about the optimal value $y^* = f(x^*)$ to measure the mutual information between $y^*$ and the next point to test
%\begin{equation}
%    MES(x) = H[p(y|\mathcal{S},x)] - E_{p(y^*|\mathcal{S})}[H[p(y|\mathcal{S},x,y^*)]].
%    \label{eq:mes}
%\end{equation}
%PESC and cMES are variants of PES and MES, respectively, which allow to take QoS constraints.

%\textcolor{red}{where we should say that these acq. func do not allow non-stationary kernels due to use of Bochner's theorem for a spectral approximation}

